Quantifying Cybersecurity Effectiveness of Software Diversity

The deployment of monoculture software stacks can cause a devastating damage even by a single exploit against a single vulnerability. Inspired by the resilience benefit of biological diversity, the concept of software diversity has been proposed in the security domain. Although it is intuitive that software diversity may enhance security, its effectiveness has not been quantitatively investigated. Currently, no theoretical or empirical study has been explored to measure the security effectiveness of network diversity. In this paper, we take a first step towards ultimately tackling the problem. We propose a systematic framework that can model and quantify the security effectiveness of network diversity. We conduct simulations to demonstrate the usefulness of the framework. In contrast to the intuitive belief, we show that diversity does not necessarily improve security from a whole-network perspective. The root cause of this phenomenon is that the degree of vulnerability in diversified software implementations plays a critical role in determining the security effectiveness of software diversity.

==> Security-effectiveness-of-natural-and-artificial-diversity.tex <==
%\subsection{Security effectiveness of natural and artificial diversity}

%In previous scenarios, we all consider the network using only one kind of operating system, namely $\OS_1$ or $\OS_2$. However, the computers in a network may use different operating system in reality, in this scenario, we would like to see the consequence after employing diversity in each operating system.
%We simulate three cases: (I) every computer runs $\OS_1$; (II) every computer runs $\OS_2$; (III) 
We consider a computer runs either $\OS_1$ or $\OS_2$ with probability 0.5. Moreover, $\OS_1$ is diversified into $N_{\OS_1}$ independent implementations and $\OS_2$ is diversified into $N_{\OS_2}$ independent implementations. We compare the case $N_{\OS_1}=N_{\OS_2}=20$ and the case $N_{\OS_1}=100$ and $N_{\OS_2}=20$.
The other parameters are: $\APP=\{$browser, email client, peer-to-peer (P2P), word processor$\}$, $C_1$ (every layer is artificially diversified), $\gamma = 0.2$ (the probability that attacks are not blocked by NIPS), $\alpha = 0.2$ (the probability that attacks that are not blocked by HIPS), $\tau(\vul) = 0.05$ (the probability that a vulnerability is zero-day), $\zeta(v)=0.5$ (the probability that $v\in V$ is vulnerable), $\capa=1$ (the attacker can exploit every vulnerability, which corresponds to the worst-case scenario), NIPS= $tight$, and HIPS= $tight$.
\begin{wrapfigure}{r}{0.25\textwidth}
%\begin{figure}[htbp!]
\centering
%\subfigure[$N_{\OS_1}=N_{\OS_2}=20$]{\label{fig:os1}
\includegraphics[width=0.23\textwidth,height=.2\textwidth]{./figures/multiple_os.pdf}
%\subfigure[$N_{\OS_1}=100$ and $N_{\OS_2}=20$]{\label{fig:os2}\includegraphics[width=0.23\textwidth,height=.196\textwidth]{./figures/multiple_os2.pdf}}
\caption{Plot of $\pca(t)$ and $\pcos(t)$ with $(N_{\OS_1},N_{\OS_2})$.}
%The straight lines represent the portion of compromisable applications or operating systems (e.g., ${|\{v:v\in V_{(app)}\vee \eta(v)\neq \emptyset\}|}/{|V_{(app)}|}$ for $\pca$.
%{\color{red}Dashed and dotted} straight lines represent the compromisable applications and operating systems, respectively.}
% with $C=C_1$, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta=0.5$, $\capa=1.0$, while using different operating systems in a network along with network diversity.}
\label{figure:natural-diversity-single-vs-multiple-os}
\vspace{-5mm}
\end{wrapfigure}

Figure \ref{figure:natural-diversity-single-vs-multiple-os} plots $\pca(t)$ and $\pcos(t)$ with respect to $(N_{\OS_1},N_{\OS_2})$.
We observe that $\pca(t)$ and $\pcos(t)$ initially increase at an exponential pace, and then converge to the a stable state. 
%However, they eventually stay below their respective maximum value (e.g., about $92\%-88\%=4\%$ in Case I with parameter combination (i)). This is because some vulnerabilities cannot be exploited remotely {\color{red}and anything else???}.
Moreover, there are always more compromised applications than compromised operating systems, because when an operating system is compromised, all of the applications running on top of it are all compromised.
We also observe that the higher the artificial diversity, the more security is gained. 
For example, we observe $\pca(100)=0.4680$ for $(N_{\OS_1},N_{\OS_2})=(20,20)$ and $\pca(100)=0.3265$ for $(N_{\OS_1},N_{\OS_2})=(100,20)$, meaning a 30\% improvement in security.
This leads to:

\begin{insight}
It is beneficial to use both natural and artificial diversity, assuming that the indpendent implementations do not incur extra vulnerabilities.
\end{insight}




==> Security-effectiveness-of-natural-diverisity.tex <==

We consider natural diversity at both the application layer and the operating system layer because they are realistic. This means $N=1$ for every application, library, kernel and driver.

We measure the security effectiveness of application-layer natural diversity by considering the case of two browsers: $\browser_1$ and $\browser_2$ (as a simplified setting for the competition between Chrome and Firefox and IE). Specifically, we consider three scenarios: (i) every computer runs $\browser_1$; (ii) every computer runs $\browser_2$; (iii) the ``hybrid'' case in where every computer runs either $\browser_1$ or $\browser_2$ with probability 0.5.
The other parameters are: $\KERNEL=\OS_2$software stack diversity configuration $C_1$ with $N=1$ (which is equivalent to $C_0$ with two browsers), $\KERNEL=\OS_1$, $\gamma = 0.2$ (the failure probability of NIPS), $\alpha = 0.2$ (the failure probability of HIPS), $\tau(\vul) = 0.05$ (the probability $\vul$ is zero-day), $\zeta(v)=0.2$ for $v\in V-\{\browser_1,\browser_2\}$ (the probability the software assigned to run at $v$
is vulnerable), $\capa=1$ (the attacker can exploit every vulnerability, corresponding to the worst-case scenario), NIPS= $tight$, and HIPS= $tight$.

\begin{figure}[htbp!]
\centering
\subfigure[$\pca(t)$ and $\pcos(t)$ with browser natural diversity]{\includegraphics[width=.23\textwidth]{./figures/broswer.pdf}\label{fig:app-layer-natural-diversity}}
\subfigure[$\pca(t)$ and $\pcos(t)$ with operating system natural diversity]{\includegraphics[width=.23\textwidth]{./figures/two_os.pdf}\label{fig:os-layer-natural-diversity}}
\caption{Plots of $\pca(t)$ and $\pcos(t)$ w/ natural diversity.}
% with $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta$=0.2, $\omega=0.15$, $\capa=1$.}
\label{mul_layer_apps}
\vspace{-2mm}
\end{figure}

Fig. \ref{fig:app-layer-natural-diversity} plots $\pca(t)$ and $\pcos(t)$ with browser natural diversity, with
$\zeta(\browser_1)=0.4$ (the probability that $\browser_1$ is vulnerable) and $\zeta(\browser_2)=0.2$ (the probability that $\browser_2$ is vulnerable).
We observe that a higher (lower) browser vulnerability probability $\zeta$ leads to a higher (lower) $\pca(t)$, and the hybrid of them leads to a $\pca(t)$ somewhere in between them.
%a higher browser vulnerability probability $\zeta$ leads to a higher $\pca(t)$
On the other hand, $\pcos(t)$ is not affected because the underlying operating system is the same.

%\noindent{\bf Effectiveness of using using single vs. multiple operating systems}.
Similarly, we measure the security effectiveness of operating system-layer natural diversity by considering the case of two operating systems: $\OS_1$ and $\OS_2$ (as a simplified setting for the competition between various kinds of Unix and Windows). We consider three scenarios: (i) every computer runs $\OS_1$; (ii) every computer runs $\OS_2$; (iii) the ``hybrid'' case in where every computer runs either $\OS_1$ or $\OS_2$ with probability 0.5.
%We simulate three scenarios: (I) every computer runs $\OS_1$; (II) every computer runs $\OS_2$; (III) every computer runs $\OS_1$ (and therefore $\OS_2$) with probability 0.5.
%First, we consider the case that $\OS_1$ and $\OS_2$ have the same mount of diversified implementations, to be specific, we set $N=20$ for each operating system. Then we employ the network with three strategies: all the computers using $\OS_1$; all the computers using $\OS_2$; all the computers using hybrid of both with each one occupies 50\%.
The other parameters are:
%We consider the following parameters: $\APP=\{$browser, email client, peer-to-peer (P2P), word processor$\}$,
browser being the $\browser_2$ mentioned above,
software stack diversity configuration $C_1$ with $N=1$ (which is equivalent to $C_0$ with two operating systems), $\gamma = 0.2$, $\alpha = 0.2$, $\tau(\vul) = 0.05$, $\zeta(v)=0.2$ for $v\in V - \{\OS_1,\OS_2\}$, $\capa=1$, NIPS= $tight$, and HIPS= $tight$.

Fig. \ref{fig:os-layer-natural-diversity} plots $\pca(t)$ and $\pcos(t)$ with operating system natural diversity, with
$\zeta(\OS_1)=0.2$ (the probability that $\OS_1$ is vulnerable) and $\zeta(\OS_2)=0.4$ (the probability that $\OS_2$ is vulnerable).
%(iii)$\zeta(\OS_1)=0.2$, $\zeta(\OS_2)=0.4$.
We observe that a higher (lower) operating system vulnerability probability $\zeta$ leads to a higher (lower) $\pcos(t)$, and the hybrid of them leads to a $\pcos(t)$ somewhere in between them.
%a higher browser vulnerability probability $\zeta$ leads to a higher $\pca(t)$
%On the other hand, $\pcos(t)$ is not affected because the underlying operating system is the same.
Note that even though when every computer runs $\OS_2$, which has a vulnerability probability $0.4$, does not necessarily mean all of the vulnerable operating system can be compromised.
This is because some vulnerabilities cannot be reached, and therefore cannot be exploited, by the attacker despite that the attacker has the corresponding exploits.

Summarying the preceding dicussion, we observe that when market competition leads to the emerge of a lower software, security is degraded  (e.g., the emergence and deployment of
$\OS_2$ with $\zeta=0.4$ causes $\pca(100)$ incareses from 0.1092 to 0.1834 in the hybrid case, meaning a $69.9\%$ security degradation).
However, if market competition leads to higher quality of software, security can be improved (e.g., the emergence and deployment of
$\browser_2$ with $\zeta=0.2$ causes $\pca(100)$ decreases from 0.5543 to 0.5314 in the hybrid case, meaning a $4.3\%$ security improvement).
It is worth mentioning that Fig. \ref{mul_layer_apps} also shows that in any case, $\pca(t)\geq \pcos(t)$ for a given parameter setting. This is because a compromised operating system causes the compromise of any application running on that computer.

\begin{insight}
Natural diversity can lead to higher security as long as the diverisified software implementations
% (emerged from market competition) 
have a higher security quality (i.e., containing fewer software vulnerabilities); otherwise, natural diversity can lead to lower security.
\end{insight}

\ignore{
\begin{figure}[htbp!]
\centering
\subfigure[$\pca(t)$]{\includegraphics[width=.23\textwidth]{./figures/two_os_pca.pdf}}
\subfigure[$\pcos(t)$]{\includegraphics[width=.23\textwidth]{./figures/two_os_pcos.pdf}}
\caption{Plots of $\pca(t)$ and $\pcos(t)$.}
% with $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta$=0.2, $\omega=0.15$, $\capa=1$.}
\label{mul_layer_os}
\end{figure}
}




==> Security-effectivness-of-artificial-diversity.tex <==
%Now we seek deeper insights.

%\newpage

\noindent{\bf Does software diversify always lead to higher security?}
%The degree of software vulnerability can be measured by the prevalence of software vulnerabilities and the attributes of the vulnerabilities, which are respectively investigated below.
We focus on $C_0$ and $C_1$ because $C_0$ in a sense reflects the state-of-the-art and $C_1$ reflects the ideal case.
The other parameters are: $\APP=\{$browser, email client, peer-to-peer (P2P), word processor$\}$, operating system is $\OS_1$, $N = 20$, $\gamma = 0.2$, $\alpha = 0.2$, $\vartheta = 0.8$, $\tau = 0.05$, $\omega=0.2$, NIPS= $tight$, HIPS= $tight$.
%In the first step, we explore whether network diversity is an effective technique to enhance the network security.
%{\color{red}We simulate two different settings:  of $C$= $\{C_0,C_1\}$, namely using monoculture implementations for each software or enforcing  multi-layer diversity for all softwares.


\begin{figure}[htbp!]
%\setlength{\abovecaptionskip}{0em}
%\setlength{\belowcaptionskip}{-1em}
%\begin{tabular}{cc}
\centering
%\subfigure[$C=C_0$, $\zeta=0.5$]{\label{fig:subfig:a}\includegraphics[width=0.23\textwidth]{./figures/no_diversity.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.5$]{\label{fig:subfig:b}\includegraphics[width=0.23\textwidth]{./figures/diversity_5.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.8$]{\label{fig:subfig:c}\includegraphics[width=0.23\textwidth]{./figures/diversity_3.pdf}}
\subfigure[$C_0$, $\zeta=0.1$]{\label{fig:subfig:a}\includegraphics[width=0.23\textwidth]{./figures/threem_2.pdf}}
\subfigure[$C_1$, $\zeta=0.1$]{\label{fig:subfig:b}\includegraphics[width=0.23\textwidth]{./figures/threem_2_1.pdf}}
\subfigure[$C_0$, $\zeta=0.1$]{\label{fig:subfig:c}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_3.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.8$]{\label{subfig:c}\includegraphics[width=0.23\textwidth]{./figures/kernel_8_1.pdf}}
\subfigure[$C_1$, $\zeta=0.1$]{\label{fig:subfig:d}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_4.pdf}}
\subfigure[$C_0$, $\zeta=0.2$]{\label{fig:subfig:e}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_1.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.8$]{\label{subfig:c}\includegraphics[width=0.23\textwidth]{./figures/kernel_8_1.pdf}}
\subfigure[$C_1$, $\zeta=0.2$]{\label{fig:subfig:f}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_2.pdf}}
\caption{Plots of $\pca$ and $\pcos$.}
% with $N = 20$, $\gamma = 0.2$, $\alpha = 0.2$, $\vartheta = 0.8$, $\tau = 0.05$, $\omega=0.2$.}
\label{diversity_2}
\vspace{-2mm}
\end{figure}
Fig. \ref{diversity_2} plot $\pca$ and $\pcos$ with respect to attacker capability $\capa$ (the fraction of vulnerabilities for which the attacker has exploits) and time. 
We observe the following. First, Figs. \ref{fig:subfig:a} and \ref{fig:subfig:c} show that monoculture $C_0$ can lead to sudden ``jumps'' in terms of compromised applications and operating systems, namely that a single vulnerability can cause the compromise of many software. The ``jumps'' are even more significant for bigger $\zeta$ as shown in Fig. \ref{fig:subfig:e} (e.g., $z=0.2$, meaning 20\% software is vulnerable). However, Figs. \ref{fig:subfig:b} and \ref{fig:subfig:d} show that the enforcement of network diversity $C_1$ does not suffer from this problem. This confirms the intuition that diversity can make the damage increases smoothly rather than abruptly. This example highlights that diversity can make the security degrades gradually rather than abruptly.

Second, suppose $\zeta$ is fixed, meaning that the security quality of independent implementations (in terms of their probabilities of containing a vulnerability) is the same. Suppose the attacker capability of the attacker $\capa$, namely the number of exploits the attacker has is proportional to the number of vulnerabilities. Figs. \ref{fig:subfig:a} and \ref{fig:subfig:b} show that $\pca(100)$ with respect to $C_0$ and $\pca(100)$ with respect to $C_1$ are almost the same, meaning that enforcing software diversity does not lead to better security. This is because increasing $N$ also increasing $N\times \zeta \times \capa$ proportionally for fixed $\zeta$ and $\capa$. This example highlights when diversity neither increase nor decreases security.

Third, by comparing Figs. \ref{fig:subfig:b} and \ref{fig:subfig:e}, we observe that diversity indeed leads to higher security when the diversified software has fewer vulnerabilities than the monoculture case. Indeed, the security resulting from diversity is almost proportional to the improvement in software quality, namely the improvement in terms of reducing $\zeta$ (the probability that a software is vulnerable) from 0.2 to 0.1. This example highlights when diversity leads to higher security.

Fourth, by comparing Figs. \ref{fig:subfig:a} and \ref{fig:subfig:f}, we observe that diversity actually can lead to worse security when the software quality in the diversified implementations is lower. Indeed, the security resulting from the use of diversified low-quality software is almost proportional to the quality of the software. For example, considering $\capa=1$ and $\pca(100)$, the damage when using lower-quality diversified software ($\zeta=0.2$) is 1.6 times of the damage of using higher-quality monoculture ($\zeta=0.1$). This example highlights that diversity actually can lead to lower security.

% compromised applications shows a "stepped" increase if there is no network diversity employed. In some interval such as $\capa\in(0.5,0.6)$ the graph is nearly flat which indicates that there is few application being newly compromised. However, in some other interval such as $\capa\in(0.6,0.7)$, a dramatic leap appears, which suggests that a large number of applications are compromised during this period. This phenomenon illustrates that the security state of the network with monoculture softwares is quite unpredictable and highly dependent on the attacker's capability, that is the exploits the attacker own. Once the attacker owns the exploit of a vulnerability existing in the network, all the hosts running this application will be the victims. On the other hand, Figure \ref{fig:subfig:b}, \ref{fig:subfig:d} present relatively smooth surfaces, which indicates that whoever the attacker is or whatever the attacker's capability might be, the security state of the network is predictable to some extent if a multi-layer diversity technique is employed on the network. The scenario that a great many applications/hosts are compromised at the same time will no happen.

%Figure \ref{diversity_2} plots the evolution of compromised operating systems in the network with the increasing of attacker's capability $\capa$ over time. The phenomenon is similar except that the compromised operating systems shows a more obvious "stepped" increase. This illustrates that there may exist several factors contributing to the compromise of applications, not only vulnerabilities in application layer, but also vulnerabilities in library layer and operating system, which make the evolution of compromised applications mitigatory comparing with the evolution of compromised operating systems.

%Besides, Figure \ref{diversity_2} shows that network diversity does not necessarily improve network security. The growing infection rate is closely related to the value of $\zeta$, namely the proportion of vulnerable implementations. To make it clear, Figure \ref{right_views} depicts the right view of each graph in Figure \ref{diversity_1} as an example. As is shown, the pink curve representing monoculture is interlaced with the green curve which represents the diversity with $\zeta$=0.5, always above the blue curve with $\zeta$=0.2 and below the cyan curve with $\zeta$=0.8. This indicates that if the proportion of vulnerable implementations is above 0.5, network security will not be enhanced by diversity, but even reduced in this scenario. However, a lower proportion of vulnerable implementations will lead to a better security state of the network.

%In summary, we have 
\begin{insight}
Network diversity can smoothen, or gradually (rather than abruptly) increase the damage when the attacker gets more powerful. However, the security effectiveness of network diversity largely depends on the security quality of the diversified software implementations, meaning that diversity can increase, make no difference, or decrease security depending on the relative quality between the diversified implementations and the monoculture implementation.
%will definitely avoid the rapidly widespread outbreaks of infection because of software monoculture and make network security state predictable, but does not definitely enhance the network security, which is highly dependent on the proportion of vulnerable implementations.
\end{insight}


\ignore{

\noindent{\bf Security  with respect to varying $\vartheta$ and $\tau$}.
After considering the most important direct factors in network diversity, we investigate some other factors that might also influence the effectiveness of diversity. First,we consider the impact of software vulnerability attributes, namely attributes $\loc$ and $\zd$ for each vulnerability exits in software.  We setup scenario instances studied here take $\APP=\{\text{browser, email client, peer-to-peer (P2P), word processor}\}$, operating system is $\OS_1$, $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\zeta=0.2$, $\omega=1$, $\capa=1.0$, $C=C_1$, NIPS= $tight$, HIPS= $tight$.

\begin{insight}
The occupation ratio of vulnerabilities that can be exploited remotely in the network will affect both the compromise rate and convergence speed against applications and operating systems. The occupation ratio of zero-day vulnerabilities
in the network will only affect the convergence speed if there does not exist a HIDS.
\end{insight}
 \begin{figure}[htbp!]
%\setlength{\abovecaptionskip}{0em}
%\setlength{\belowcaptionskip}{-1em}
%\begin{tabular}{cc}
\centering
\subfigure[impact of $\vul$ attribute of $\loc$]{
\label{vul_loc}
\includegraphics[width=0.23\textwidth,height=.2\textwidth]{./figures/loc.pdf}}
\subfigure[impact of $\vul$ attribute of $\zd$]{
\label{vul_zd}
\includegraphics[width=0.23\textwidth,height=.2\textwidth]{./figures/zd.pdf}}
\caption{Plot of $\pca(t)$ and $\pcos(t)$ with $C=C_1$, $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\zeta=0.5$, $\omega=0.2$, $\capa=1.0$,  changing vulnerability attributes $\vartheta$ and $\tau$. }
\label{vul}
\vspace{-2mm}
\end{figure}

In order to investigate the impact of $\vartheta$, we set $\tau=0.05$ which means that around 5\% vulnerabilities in the network are zero-day vulnerabilities. We observe the evolution of compromised applications and compromised operating systems with different settings of $\vartheta\in\{0,0.5,1.0\}$ as shown in Figure \ref{vul_loc}, the value of $\vartheta$ will affect both the infection speed and final infection rate. To be specific, the higher the proportion of vulnerabilities that can be exploited remotely in the network, the faster and the more applications and operating systems will be compromised. This is owing to the fact that remote exploitation is always the main channel to make lateral movement.

In order to investigate the impact of $\tau$, we fix $\vartheta=1.0$ to observe the evolution of application infection rate with different settings of $\tau\in\{0,0.5,1.0\}$. As we can see from Figure \ref{vul_zd}, a higher proportion of zero-day vulnerabilities will lead to a drastic compromise speed, while the final compromised applications and compromised operating systems remain unaffected. The rapid compromise speed is mainly due to the feature of zero-day vulnerabilities, namely that they can not be prevented by any intrusion prevention system. The main reason why more zero-day vulnerabilities do not cause more applications compromised is on account of the precondition of our scenario, that is there does not exist a HIDS in each computer which means once a application is compromised it will no longer be detected and recovered. On the other hand, $\alpha>0,\gamma>0$ indicates that a attacker can always try many times until breaking through the intrusion prevention system and compromise the node, and the P2P clients make the attacks more intense.

}


\noindent{\bf Is the resulting security linear to the degree of diversity $N$ when diversity indeed improves security?}
Suppose the attacker has a fixed number of exploits, say $|X|=4$. 
Because enforcing diversity at all layers ($C_1$) leads to a higher security, we now investigate 
\begin{wrapfigure}{r}{0.25\textwidth}
\centering
{\includegraphics[width=0.23\textwidth,height=0.2\textwidth]{./figures/versions.pdf}}
\caption{$\pca(100)$ and $\pcos(100)$.}
% with $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta$=0.2, $\omega=1$ , $\capa=0.2$,$t=100$}
\label{versions}
\end{wrapfigure}
the effect of $N$, $\omega=1$ (100\% nodes of $\Weapon$ are initially compromised), $\gamma = 0.2$, $\alpha = 0.2$, $\vartheta = 0.8$, $\tau = 0.05$, $\zeta=0.2$, $\capa=0.2$, and $t=100$.
%while keeping the other parameters the same as in Fig. \ref{mul_layer_apps}. 
%In previous scenarios we have investigated the whether network diversity is effective and which diversity strategy is more effective. Now we consider the impact of diversity effort, that is the number of varying diversified implementations. We setup scenario instances studied here as $\APP=\{\text{browser, email client, peer-to-peer (P2P), word processor}\}$, $\KERNEL$= $\OS_1$, $C=C_1$, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta=0.2$, $\omega=1$,NIPS= $tight$, HIPS= $tight$. We assume that the attacker owns all the exploits for $N=20$, namely the attacker's capability is limited, and analyzed security gain by taking
%\begin{figure}[htbp!]
Fig. \ref{versions} plots $\pca(100)$ and $\pcos(100)$ with varying $N$. We observe that when $N\leq20$, increasing $N$ does not lead to any significantly better security in terms of the two metrics, because when $N\leq 20$, each layer has no more than $0.2\times 20=4$ vulnerabilities, which can all be exploited.
When $N>20$, increasing $N$ does lead to better security because the attacker has only 4 exploits or exploit 4 vulnerabilities, even though there are for $N=100$, $0.2\times 100=20$ vulnerabilities at a single layer.
%Note that in the setting with $\capa=0.2$, $\zeta=0.2$ and $N=100$, the attacker can exploit on average $0.2\times 0.2\times 100=4$ vulnerabilities at a layer; in the setting with $\capa=1.0$, $\zeta=0.2$, and $N=20$, the attacker can exploit on average $1\times 0.2 \times 20=4$ vulnerabilities at a layer.
We further observe that security effectiveness, namely $1-\pca(100)$ and $1-\pcos(100)$, increases faster when $N\in [20,60]$ than $N\in[60,100]$.
This manifests a kind of ``diminishing return.'' Therefore, we have
%also notice that the rate of decline is not constant, fast at first but then slow down gradually. The morphology seems to be a convergent adaptation, which means that given a network there might exist a certain threshold value of $N$, under which the network diversity is effective and efficient, but beyond which the extra security gain is limited, even negligible.

\begin{insight}
Given a fixed attack capability in terms of the exploits to the attacker, increasing $N$ (diversity effort) leads to better security only when some vulnerabilities cannot be exploited by the attacker. Moreover, there is a ``diminishing return'' in terms of the security effectiveness, suggesting the existing of an optimal or cost-effectiveness $N$.
\end{insight}



\noindent{\bf How to prioritize software diversity at the layers when diversity indeed improves security?}
Recall that configuration $C_0$ means monoculter, $C_1$ means enforcing diversity at all three layers, and $C_2,C_3,C_4$ respectively mean enforcing diversity at the application, library, and operating system layer. For comparing their effectiveness, we consider the following parameters: $\APP=\{$browser, email client, peer-to-peer (P2P), word processor$\}$, operating system is $\OS_1$, $\zeta=0.2$ (20\% software has a vulnerability), $\tau = 0.05$ (5\% vulnerabilities are 0-day), $\capa=1.0$ (the attacker can exploit all vulnerabilities), $N = 20$ (in the case of $C_1,\ldots,C_4$), $\gamma = 0.2$ (NIPS failure probability), $\alpha = 0.2$ (success probability of social engineering attack), $\vartheta = 0.8$ (i.e., 80\% vulnerabilities can be exploited remotely), $\omega=0.15$ (15\% nodes of $\Weapon$ are initially compromised), NIPS= $tight$, and HIPS= $tight$.

\begin{figure}[htbp!]
\centering
\subfigure[$\pca(t)$]{\includegraphics[width=.23\textwidth]{./figures/diversity_app.pdf}}
\subfigure[$\pcos(t)$]{\includegraphics[width=.23\textwidth]{./figures/diversity_kernel.pdf}\label{multiple_layer_kernel}}
\caption{$\pca(t)$ and $\pcos(t)$.}
% with $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta$=0.2, $\omega=0.15$, $\capa=1$.}
\label{mul_layer_apps}
\vspace{-2mm}
\end{figure}
Fig. \ref{mul_layer_apps} plots $\pca(t)$ and $\pcos(t)$.
We observe that for the same configuration and parameters, $\pca(t)>\pcos(t)$ for any $t$. This means that there are more compromised applications than compromised operating systems.
Moreover importantly, we observe that metric $\pca(t)$ shows $C_0 \prec C_3 \prec C_4 \prec C_2 \prec C_1$ but metric $\pcos(t)$ shows $C_0 \prec C_3 \prec C_2 \prec C_4 \prec C_1$, where $C_a \prec C_b$ means configuration $C_b$ leads to a higher security than $C_a$. 
For example, $\pca(100)$ for $C_0$ is 2.86 times of $\pca(100)$ for $C_1$, meaning that enforcing diversity at all three layers can reduce 65\% of the damage when compared with the case of monoculture. This leads to:

\begin{insight}
When diversity can improve security, enforcing diversity at multiple layers leads to higher security than enforcing diversity at a single layer. and enforcing diversity at the operating system layer leads to higher security than enforcing diversity at the application layer, which is better than the library layer. 
%Enforcing diversity is always better than monoculture.
\end{insight}


\ignore{

\noindent{\bf Effectiveness against varying degree of initial compromise}.
%As discussed before, in order to penetrate into the network, the attacker needs to initial compromise some applications as "stepping stones" to attack other computers. Now we consider the the extra cost of the attacker needs to pay to achieve a certain gain by using network diversity.  We setup scenario instances studied take.
Fig. \ref{initial_compromise} plots $\pca(100)$ and $\pcos(100)$ with respect to varying $\omega$ (the fraction of nodes in $\Weapon$ that are initially compromised by the attacker) and different $\capa$'s, while noting that the other parameters are: 
$\APP=\{$browser, email client, peer-to-peer (P2P), word processor$\}$, operating system is $\OS_1$, $N = 20$, $\gamma = 0.2$, $\alpha = 0.2$, $\vartheta = 0.8$, $\tau = 0.05$, $\zeta=0.2$, NIPS= $tight$, HIPS= $tight$, and $T=100$.

% the changing of compromised applications and compromised operating systems with regard to initial compromise rate. We can make the following observations. First, the compromised rate is increasing fast at the beginning and then slow down gradually for both software monoculture and network diversity, which means that lateral movement is more frequent at start for both. Second, the percentage of compromised applications($\pca$) and compromised operating systems($\pcos$) of mutliple-layer diversity are always lower than that of software monoculture even if the attacker has used more exploits, this is because network diversity has expand the required exploits set that needed to compromise all the vulnerable softwares. In other words, the attacker cost more, but get less reward.Third, mutliple-layer diversity nearly stopped changing after the initial compromise rate comes to approximate 0.3, which means that the attacker can use less initial compromise make more lateral movements and achieve the most reward in the case of software monoculture, which is  frustrating for the defender, this maybe due to the fact that the network diversity has cut these connected subgraphs into many smaller subgraphs that the attacker can reach based on the exploits the attacker owns.

\begin{figure}[htbp!]
\centering
\subfigure[$\pca(100)$]{\includegraphics[width=0.23\textwidth,height=0.2\textwidth]{./figures/initial.pdf}}
% with $C=C_1$, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta=0.5$, $\capa=1.0$, while using different operating systems in a network along with network diversity.}
\subfigure[$\pcos(100)$]{\label{}\includegraphics[width=0.23\textwidth,height=0.2\textwidth]{./figures/initial2.pdf}}
\caption{Plot of $\pca(100)$ and $\pcos(100)$ with respect to $\omega$.}
% when $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\vartheta$ = 0.8, $\tau$ = 0.05, $\zeta=0.2$ ,$T=100$.}
\label{initial_compromise}
\vspace{-2mm}
\end{figure}

%Since we use the tight network access control policy, which means that any communication that is not specified will be blocked. In other words, the network $G$ is consisted of several connected graphs. For each initial compromised application, the attacker can make lateral movements to compromise the application in the connected subgraph it locates in, but can not comprise the applications in other subgraphs even if the attacker has the exploits.
We observe that $\pca(100)$ for $C_0$, $C_0, cap=25\%$ is the worst case, $C_0, cap'=25\%$ is the random(average) case. We assume the attacker will randomly choose a vulnerable application as the initial compromised node, until all the applications can be initial compromised are traversed.

\begin{insight}
Software monoculture may cost less, but get more reward, however network diversity requires the attacker costs more, but gain less.
\end{insight}


}






























==> attacker_consequence_description.tex <==
%\subsubsection{Representation of software states}

%Recall that in order to make the model as realistic as we can, proposed dividing the software stack of a computer into three layers: the {\em application} layer, the {\em library} layer, and the operating system (i.e., {\em kernel} and {\em driver}) layer. Recall also that in order to model cyber attacks as realistic as we can, we further proposed modeling these layers at a finer granularity: the library layer contains multiple libraries, with each library containing multiple library functions; the kernel contains multuple kernel functions; there are multiple drivers, with each containing multiple driver functions. Correspondingly, we defined the mathematical function $\compromised:V\in \{0,1\}$ in \eqref{eq:node-state-definition} to represent the security state of $v\in V_{(app)}\cup V_{(os)}$, while noting that no security state is defined for a library function because it is always loaded into the address space of an application at runtime. 

%In order to measure the security state of a network, we propose measuring the security state of an operating system. Naturally, an operating system is compromised if any kernel or driver function is compromised; moreover, any application running on top of the operating system is compromised. Rather than introducing a new notation, we can extend the the mathematical function $\compromised$ as defined in \eqref{eq:node-state-definition} to represent the state of an operating system running in computer $i$. Let $\driver_{i}=\cup_j \driver_{i,j}$ be the set of driver functions running in computer $i$. 

The attack consequence is represented by the predict of $\state(v)$ of $v\in V$. Given the state of a kernel or driver, we can define the state of an operating system as
%Then, we can define the security state of an operating system as:
\begin{eqnarray*}
%\compromised(\app_{i,j}) &= &\compromised(\app_{i,j}) \\
%\compromised(\kernel_{i}) &= &\bigcup_{k_{i,z}\in \kernel_{i}}\compromised(k_{i,z})\\
%\compromised(\driver_{i,j}) &= &\bigcup_{d_{i,j,z}\in \driver_{i,j}}\compromised(d_{i,j,z})\\
\state(os_i) = 
\left\{
\begin{array}{ll}
1 & \exists v\in \kernel_i \vee \driver_{i}~\text{s.t.}~\state(v)=1 \\ 
0 & otherwise
\end{array}
\right.
\end{eqnarray*}
Moreover, we have
\begin{eqnarray*}
\forall \app_{i,j}\in V_{i,app}: \state(os_i)=1 \Longrightarrow \state(\app_{i,j})=1.
\end{eqnarray*}


==> case-study.tex <==

\subsection{Simulation setup and method}
\label{sec:network_attack_defense_setting}

\input{network_attack_defense_setting.tex}


\input{case_study_beta_0.tex}

\subsection{Seeking deeper insights into software quality}

\input{seeking-deeper-insights.tex}

\subsection{Regression Analysis}
\label{sec:regression-analysis}
\input{regression-analysis.tex}

 



==> framework.tex <==
%It is intuitive that enforcing network diversity may enhance network security from a whole-network perspective. However, an important problem that has not been addressed is: {\em How can we quantify the security effectiveness of enforcing network diversity?}
%{\color{blue}How can we maximize the security gain by optimizing the network diversity?}
\comb{To} quantify the effectiveness of network diversity \comb{on security}, we propose the framework in in Fig. \ref{fig:framework}, \comb{which} describes: (1) how to abstract a network, its vulnerabilities, its defenses, and its software stacks; (2) how to represent attacks; (3) how to represent \comb{the consequences (i.e., impact) of} the attack; (4) how to define security metrics; and (5) how to compute the effectiveness \comb{of software diversity on system security}.
%It is clear that this framework should single out the factor that describes the network diversity. This factor is called {\em software stack configuration}.
%The distinction between the network security configuration in the physical network and the abstract representation makes the framework clean.
%But other factors that need to be adequately abstracted as well.
\begin{figure}[!htbp]
\centering
\includegraphics[width=.46\textwidth]{./figures/framework_final.pdf}
\caption{The framework \comb{that quantifies} the effectiveness of network diversity \comb{on system security}.
%{\color{blue}If we do not deal with optimization in this paper, we need to simplify the picture}
\label{fig:framework}}
\end{figure}
%The framework is composed of of six components, which are briefly mentioned below and will be elaborated in the next subsections.
%The first component is responsible for abstracting an enterprise network into some appropriate representation. The representation includes two kinds of relations: the {\em communication} relation describing which computer can or cannot communicate with which other computer (as regulated by firewall rules), and the {\em dependence} relation describing which software component calls which other software component.
%(e.g., a vulnerability in the kernel can cause the compromise of the computer running the corresponding operating system).
%The second component is responsible for abstracting the configuration of software stacks, such as which computer installs which version of the software components.
%The third component is responsible for abstracting attacks, such as the attacker vectors that are available to the attacker.
%The four component is responsible for abstracting the attack consequences.
%The fifth component is for defining security metrics of interest.
%The sixth component is for computing the security metrics with respect to specific attacks against defenses in specific enterprise networks, and to generating instructions on how to enhance the security of the enterprise network.

At a high-level, let $G$ represent a network \comb{(e.g., an enterprise network)}, $A$ represent the attacks against the network, $B$ represent the vulnerabilities of the network's software systems and human factors, $C$ represent the software stack configuration of the network, $D$ represent the defenses to protect the network, and $M=\{m_i\}$ represent a set of security metrics of interest. Let us ignore for a moment how $G$, $A$, $B$, $C$, $D$ and $M$ will be represented. In principle, there exists a family of mathematical \comb{functions} $\{{\cal F}_i\}_i$ for computing the network's security in terms of metric $m_i\in M$, namely
\begin{equation}
\label{eq:framework-equation}
m_i={\cal F}_i(G,A,B,C,D).
\end{equation}
Intuitively, $m_i$ reflects the outcome of the interaction between attacks $A$ and defenses $D$ in a network $G$ with software stack configuration $C$ and vulnerabilities $B$.
%In general, this abstraction allows us to compare the security incurred by two networks, say $G_1$ and $G_2$, and/or two attackers, say $A_1$ and $A_2$, and/or two software stack configurations, say $C_1$ and $C_2$, and/or two defenses, say $D_1$ and $D_2$.
Therefore, we can quantify the security effectiveness of \comb{network} diversity by comparing the security respectively incurred by software stack configurations, say $C_1$ and $C_2$, namely
$$
{\cal F}_i(G,A,B,C_1,D) ~~~\text{and}~~~ {\cal F}_i(G,A,B,C_2,D)
$$
for every ${\cal F}_i$ (i.e., for every metric $m_i\in M$ of interest).
\comb{In this work, we} seek \comb{to rigorously represent} $G$, $A$, $B$, $C$ and $D$, \comb{define} security metrics $m_i$'s, and ideally and explicitly express the mathematical functions ${\cal F}_i$'s. These issues are described in the rest of the \comb{this} section.

\ignore{
\subsubsection{Methodology}

For this purpose, we define a tuple of functions
\begin{equation}
\label{eq:tuple-of-functions}
C=(C_{(app)},C_{(lib)},C_{(os)}),
\end{equation}
where
\begin{itemize}
\item $C_{(app)}: V_{(app)} \to \APP^{(N)}$ is the function for assigning a specific implementation of an application $\app_{i,j}\in\APP^{(N)}$ to run at node $v\in V_{i,app}$ according to some strategy.
\item $C_{(lib)}: V_{(lib)} \to \LIB^{(N)}$ is the function for assigning a specific implementation of a library $\lib_{i,j}\in\LIB^{(N)}$ to run at node $v\in V_{i,lib}$ according to some strategy.
\item $C_{(os)}: V_{(os)} \to \KERNEL^{(N)}\cup \DRIVER^{(N)}$ is the function for assigning a specific implementation of a kernel function $\kernel_{i}^{(N)}\in \KERNEL^{(N)}$ to run at node $\kernel_i$
or a specific implementation of a driver function $\driver_{i,j}\in\DRIVER^{(N)}$ to run at a node $\driver_{i,j}\in V_{j,z}$.
\end{itemize}
}
\comb{The key notations are summarized} in Table \ref{table:notations}.
\begin{table}[!htbp]
\centering
\begin{tabular}{|l|p{.36\textwidth}|}
\hline
%$G=(V,E)$     & A directed graph represents a network of $n$ computers, where $V=V_1 \cup \ldots \cup V_n$ with $V_i=V_{i,app}\cup V_{i,lib} \cup V_{i,os}$ being the node set representing the software components in computer $i$, $E=E_1 \cup \ldots \cup E_n \cup E_0\cup E_*$ with $E_i$ being the arc set corresponding to computer $i$, $E_0$ being the inter-computer communication relation such that $(\app_{i,z}, \app_{j,z'}) \in E_0$ means the $z$-th application, denoted by $\app_{i,z}$, running in computer $i$ can communicate with the $z'$-th application, denoted by $\app_{j,z'}$, running in computer $j$ (otherwise, the traffic will be filtered), $E_*=E_{*,io}\cup E_{*,oi}$ being the arc set representing the internal-external communication relations such that $E_{*,io}=\{(\app_{i,1},*)\}$ meas $\app_{i,1}$ can communicate with any computer ``$*$'' that resides outside of the network, $E_{*,oi}=\{(*,\app_{j,1})\}$ means that any computer ``$*$'' outside the network can communicate with $\app_{j,1}$.\\
%$B$           & $B $ denotes the set of all vulnerabilities that exist in the network.\\
%$G_i$           & directed graph $G_i=(V_i,E_i)$ correspond to  computer $i$, where vertex set $V_i=V_{i,app}\cup V_{i,lib} \cup V_{i,os}$ represents the software components in computer $i$ and arc set $E_i=E_{i,a}\cup E_{i,l}\cup E_{i,al}\cup E_{i,lk} \cup E_{i,ak}\cup E_{i,ad}$ describes the dependence and communication relations between the relevant software components.\\
application & $\APP$ is the universe of applications; $\eta: \APP \to  \{0,1,2\}$ indicates the type of an application (client vs. server vs. other); $\app_{i,z}\in \APP$ is the $z$-th application running \comb{on} computer $i$\\
\hline
library & $\LIB$ is the universe of libraries; $\lib_{i,j}\in \LIB$ is the $j$-th library running \comb{on} computer $i$; $f_{i,j,z}\in \lib_{i,j}$ is the $z$-th library function in $\lib_{i,j}$\\
\hline
kernel         & $\KERNEL$ is the universe of kernels; $\kernel_{i}\in \KERNEL$ is the kernel running \comb{on} computer $i$; $k_{i,z}\in \kernel_{i}$ is the $z$-th kernel function in $\kernel_{i}$\\
\hline
driver         & $\DRIVER$ is the universe of drivers; $\driver_{i,j}\in \DRIVER$ is the $j$-th driver running \comb{on} computer $i$; $d_{i,j,z}\in \driver_{i,j}$ is the $z$-th driver function in $\driver_{i,j}$\\
\hline
$G_i$      & $G_i=(V_i,E_i)$ represents a computer; $V_{i}=V_{i,app} \cup V_{i,lib} \cup V_{i,os}$; $E_i=E_{i,a}\cup E_{i,l} \cup E_{i,al} \cup E_{i,lk} \cup E_{i,ak} \cup E_{i,kd}$ \\
\hline
$G=(V,E)$	& $G$ represents a network of $n$ computers, where $V=V_1\cup \ldots \cup V_n$ and $E=E_1\cup \ldots \cup E_n \cup E_0 \cup E_*$\\
\hline
diversity    & $Y^{(N)}$ is the universe of diversified implementations of $Y\in \{\APP,\LIB,\KERNEL,\DRIVER\}$; $N_Z$ represents the number of independent implementations of $Z$\\
\hline
%$\APP^{(N)}$    & the universe of diversified implementations of the applications (i.e., the union of the sets representing the diversified implementations of the applications).\\
%$\LIB^{(N)}$    & the universe of diversified implementations of the libraries. \\
%$\KERNEL^{(N)}$ & the universe of diversified implementations of the kernels.\\
%$\DRIVER^{(N)}$ & the universe of diversified implementations of the drivers.\\
vulnerability & $B$ is the universe of software vulnerabilities; $\phi(v)\subseteq B$ is the set of vulnerabilities a node $v\in V$ contains;
%$|\phi(v)=0|$ means $v$ is not vulnerable;
$\zd(\vul)$ indicates $\vul\in B$ is known (`0') or zero-day (`1'); $\loc(\vul)$ indicates $\vul$ can be exploited remotely (`1') or not ('0'); $\priv(\vul)$ indicates the exploitation of $\vul$ causes the attacker to obtain the {\tt root} privilege (`1') or not ('0'); $\psi(v)$ for $v\in V_i$ is the probability that the user of computer $i$ is vulnerable to social engineering attacks \\
\hline
%$\psi$      &$\psi: V\to \{0,1\}$ describes whether $v\in V$ is not subject to social engineering attacks such that  $\psi(v)=0$ means that $v$ is not subject to those attacks enabled by human factor vulnerabilities and $\psi(v)=1$ means that $v$ will be a victim of these social engineering attacks.\\
$\gamma$    & $\gamma\in [0,1]$ is the failure probability of network-based intrusion prevention mechanism; $\gamma_{(\app_1,\app_2)}\in [0,1]$ is the failure probability in blocking attacks from $\app_1$ to $\app_2$; $\gamma_{(*,\app)}\in [0,1]$ is the failure probability in blocking inbound attacks\\
\hline
$\alpha$   & $\alpha(v) \in [0,1]$ is the failure probability that a social engineering attack against $v$ is not blocked \\
%$\beta_{i}$    & $\beta_{i}\in [0,1]$ describes the probability that the reactive defense system does not detect a successful attack against computer $i$ that does not compromise the reactive defense system. \\
\hline
$\state(v,t)$ & \comb{The} probability $v\in V_{(app)}\cup V_{(os)}$ is compromised at time $t$\\
exploit       & $X$ is the set of exploits available to the attacker; $\rho(x,\vul)$ is the probability that $x\in X$ can exploit vulnerability $\vul\in B$\\

%$C$           & $C=(C_{(app)},C_{(lib)},C_{(os)})$ is a tuple of functions that define the alternative assign of each software program with a specific implementation.\\
\hline
metrics       & $M=\{m_i\}$ is a set of security metrics\\\hline
simulation    & $\zeta(v)$ is the probability that a software running at $v\in V$ or simply $v\in V$ is vulnerable; $\capa$ is the percentage of software vulnerabilities for which the attacker has exploits; $\tau(\vul)$ is the probability that $\vul\in B$ is zero-day; $\vartheta(\vul)$ is the probability $\vul\in B$ is remotely exploitable\\\hline
\end{tabular}
\caption{Summary of notations.\label{table:notations}}
\end{table}


==> regression-analysis.tex <==
As mentioned above, an important research goal is to obtain Eq. \eqref{eq:framework-equation}, namely
$m_i={\cal F}_i(G,A,B,C,D)$.
%where $G$, $A$, $B$, $C$ and $D$ are all respectively described by a set of parameters.
%While this formulates a new way of thinking, it also means that there is no real-world data that can be readily used for this purpose.
Due to the lack of real data, 
%which might not be available for a long period of time, 
we use, as a first step, {\em linear regression} to extract Eq. \eqref{eq:framework-equation} from the simulation data with respect to $t=100$ (i.e., the stable state) and both natural and artificial diversities. 
As a result, we can quantify the influence of each factor on $\pca$ and $\pcos$ and prioritize the factors that should be paid most attention in improving security.

% lists the dependent variables $\pca$ and $\pcos$ and the explanatory variables $x_1,\ldots,x_{14}$. The variables are Specifically, we want to know how $x_1$($\OS$, the proportion of computers using $\OS_1$), $x_2$($|\APP|$, the applications using in each computer), $x_3$($\browser$, the proportion of computers using $\browser_1$, $\browser_1=0$ means all the computers using $\browser_2$), $x_4$($N$, the number of various independent implementations of each software), $x_5$($C$, each layer is artificially diversified), $x_6$($\zeta(v)$, the probability that $v\in V$ is vulnerable), $x_{7}$($\vartheta(\vul)$, the probability that a vulnerability can be remotely exploited), $x_{8}$($\tau(\vul)$, the probability that a vulnerability is zero-day), $x_{9}$($\capa$, the percentage of software vulnerabilities for which the attacker has exploits), $x_{10}$($\omega$, the percentage of vulnerable softwares chosen as initial compromise by the attacker), $x_{11}$($\alpha$, the probability that attacks that are not blocked by HIPS), $x_{12}$ ($\gamma$, the probability that attacks are not blocked by NIPS), $x_{13}$(NIPS, the probability that the NIPS enforce tight access control policy), $x_{14}$(HIPS, the probability that the HIPS enforce tight access control policy).


\begin{table}[!htbp]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
%\multirow{2}{*}{factors}      & \multicolumn{2}{c|}{security metrics}\\  \cline{2-2} \cline{3-3}
\multirow{2}{*}{parameter} &\multirow{2}{*}{meaning}     &$\pca$          &$\pcos$  \\  \cline{3-3} \cline{4-4}
         &         &$a_i$          &$b_i$                  \\ \hline
$x_1$ & fraction of $\OS_1$ in network     & -0.075043702 & -0.087896035 \\ \hline
$x_2$ & \# apps running on a computer     & 0.088058394  & 0.100100406  \\ \hline
$x_3$ &fraction of $\browser_1$ in network   &0.030891731  & 0.021767411  \\ \hline
$x_4$ &$N$   & -0.135383659 & -0.132493806 \\ \hline
$x_5$ &(see text for explanation)      & 0.052487618  & 0.06748197  \\ \hline
$x_6$ &$\zeta\in [0,1]$   & 0.134058106  & 0.191438008  \\ \hline
$x_{7}$ &$\vartheta\in [0,1]$       & 0.329777951 & 0.195278642 \\ \hline
$x_{8}$ &$\tau\in [0,1]$      & 0.034082301  & -0.011789413 \\ \hline
$x_{9}$ &$\capa\in[0,1]$     & 0.730355341  & 0.593024     \\ \hline
$x_{10}$ &$\omega\in[0,1]$   & 0.170030437  & 0.087308202  \\ \hline
$x_{11}$ &$\alpha\in [0,1]$      & 0.050954275 & 0.05991885  \\ \hline
$x_{12}$ &$\gamma\in [0,1]$  &0.0001      &0.0001      \\ \hline
$x_{13}$ &NIPS=1 (i.e., {\em tight})   & -0.049658866  &- 0.035677049  \\ \hline
$x_{14}$ &HIPS=1  (i.e., {\em tight})        & -0.037981492 & -0.310823403 \\ \hline
\end{tabular}
\caption{Description of
the explantary variables
%$\OS$ , $|\APP|$, NIPS, HIPS, $N$, $C$, $\capa$, $\zeta$, $\vartheta$, $\tau$, $\alpha$, $\gamma$) by linear models.
and the dependent variables $\pca$ and $\pcos$.}
\label{table:regression}
\end{table}

For regression, we use the 14 explanatory variables $x_1,\ldots,x_{14}$ that are listed and explained in Table \ref{table:regression}, except for $x_5$ which is determined as follows:
$C_0,C_1,C_2,C_3,C_4$ respectively corresponds to $x_5=5,1,3,4,2$. This can be justified by the decreasing order of $\pcos(100)$ as shown in Fig. \ref{multiple_layer_kernel}, namely
$C_0,C_3,C_2,C_4,C_1$. 
For the explanatory variables that are not defined over $[0,1]$, we first standardize and centralize them into $[0,1]$.
The data consists of 568 rows of these variables as well as the corresponding $\pca(100)$ and $\pcos(100)$.
Because 7 (out of the 14) variables are highly correlated with each other (e.g., the Pearson correlation coefficient between $x_5$ and $x_9$
%Cor($C$, $\capa$)=
is -0.3148, the coefficient between $x_6$ and $x_{10}$ is
%Cor($\zeta$, $\omega$)= 
0.4034, the coefficient between $x_{14}$ and $x_8$
%Cor(HIPS, $\zd$)=
is -0.45) and the amount of data is relatively small when compared with the number of variables (i.e., 14), we use the {\em partial least squares} method \cite{tobias1995introduction} to estimate the regression coefficients.
Since it should be the case that $\pca(100)=\pcos(100)=0$ when $x_1=\ldots=x_{14}=0$, the regression results are:
\begin{eqnarray}
\label{eq:regression}
\pca=\sum_{i=1}^{14}a_i x_i~~\text{and}~~\pcos=\sum_{i=1}^{14}b_i x_i,
\end{eqnarray}
where the $a_i$'s and $b_i$'s are respectively given in the 3rd and 4th column of Table \ref{table:regression}.
The cumulative R-square of $\pca(100)$ and $\pcos(100)$ in the fitted models is respectively 0.78 and 0.75, which means that the model fitting is accurate.

Table \ref{table:regression} allows us to observe the following. 
On one hand, the factors that have a significant influence on $\pca$ are $x_4, x_6,x_7,x_9,x_{10}$. 
The most significant factor is $x_9$, namely the fraction of vulnerabilities that can be exploited by the attacker. This suggests that the most significant strategy to improve application-layer security is to reduce the fraction of vulnerabilities that can be exploited by the attacker.
On the other hand, the factors that have a significant influence on $\pcos$ are $x_2,x_4,x_6,x_7,x_9,x_{14}$. 
The most significant factor is $x_{14}$, namely the tightness of NIPS. This suggests that the most significant strategy to improve operating system-layer security is to enforce tight HIPS, namely to preventing unauthorized applications, even if compromised, from waging privilege escalation attacks. 

%our models fit good. From the coefficients $a_i$ and $b_i$, we can observe the exact different impact each parameter exerts on the security state of the network with regard to $\pca$ and $\pcos$. First, we can observe that some variables are positive associated while some others are negative associated, namely the changing of some parameter may undermine the security while some others can contribute to improving network security. For example, the values of $\OS$, $N$, NIPS, HIPS are negative, which means that such defense techniques will do benefit for the defender. For example, $tight$ access control of HIPS is very effective in protecting operating system. Second, from the absolute values of $a_i$ and $b_i$, it is obvious that the effect of some parameters are more significant than others, such as attacker's capability $\capa$, the initial compromise radio $\omega$, software vulnerable probability $\zeta$, defender's effort on diversity(the number $N$ of independent implementations for a software), the vulnerabilities that can be exploited remotely $\vartheta$ , the applications running in each computer $|\APP$|. In order to enhance the network security, these factors should be a priority for consideration. Besides, the effect of $\gamma$ is so little, even negligible, which means that in a local network, NIPS/NIDS needs to keep in a rather low failure rate, otherwise it is useless in preventing the spread of virus, because all the computers can communicate with each other at one time in the same sub-network.
%However, using all the 12 independent variables may cause the overfitting problem. Moreover, linear regression model may not be able to represent specific relationships existing in our data. For example, the coefficients $a_i$ and $b_i$ of $\tau$ are unreasonable, however the zero-day vulnerability will not affect the final value of $\pca$ and $\pcos$ if there does not exist a HIDS.




==> related-work.tex <==
%The damage of software monoculture is easy to understand because a single vulnerability in a software can cause a rapid compromise of all those computers that run the software \cite{Geer2003,Stamp:2004:RM:971617.971650,zhang2001heterogeneous}. Increasing software diversity has been proposed to solve this problem by generating various programs to mitigate attacks. There has been a lot of substantial work on different techniques of automatically producing diversity. We briefly summarize previous work on different types of software diversity and frameworks in place.

Software diversity has been advocated for achieving higher security \cite{Geer2003,Stamp:2004:RM:971617.971650,zhang2001heterogeneous}. 
However, diversity, such as N-version programming \cite{avizienis1985n,chen1978n}, was originally proposed to enhance fault tolerance under the assumption that software faults occur {\em independently} and {\em randomly}. Unfortunately, this assumption does not hold because programmers may make the same mistakes \cite{knight1986experimental}, and because
because attacks are specifically geared towards software vulnerabilities (i.e., attacks are neither independent nor random). This means that the security value of enforcing software diversity must be re-examined in realistic threat models. To the best of our knowledge, the present study is the first effort aiming at systematically quantifying and characterizing the security effectiveness of software diversity. Indeed, we show that in contrast to its fault-tolerance effectiveness, network diveristy does {\em not} necessarily improve security in the plausible scenarios that the diversified implementations have the same security quality as the monoculture software implementation (i.e., containing the same amount of vulnerabilities). The misperception of diversity can improve security can be attributed to the {\em independence} assumption, which is reasonable for fault-tolerance but not for security.
This is reminiscent of a recent study in a different context of security \cite{XuInternetMath2015Dependence}, which shows that the results can be misleading when dependence is assumed away.

The most closely related prior work is \cite{ODonnellCCS2004}, which investigates how to configure diversified software implementations to the computers. Their goal is to minimize the number of neighboring nodes that have the same software implementation, and/or maximize the number of subnetworks that run the same software. This explains that \cite{ODonnellCCS2004} is algorithmic in nature. Unlike \cite{ODonnellCCS2004}, our work has the following unique perspectives: (i) our work aims to quantify the security effectiveness of enforcing network diversity, leading to insights that are not known until now; (ii) our technical approach is novel by taking a systematic system-level approach; and (iii) our mode has a finer granuality than \cite{ODonnellCCS2004}.
 
Loosely related to the present study, we mention proposals for runtime diversity,
including address space randomization \cite{bhatkar2003address,forrest1997building,etoh2000gcc,xu2003transparent}, instruction set randomization~\cite{kc2003countering,barrantes2003randomized},
and randomizing system calls \cite{chew2002mitigating}. 
Effectiveness and weakness of there techniques has been analyzed in \cite{shacham2004effectiveness,sovarel2005s}. 
Because these diversity techniques are complementary to software diversity, which is the focus of the present work, the present framework may be extended to investigate the security effectiveness of these techniques as well.
Moreover, researchers have proposed the notion of N-variant systems to achieve higher assurance in detecting attacks~\cite{cox2006n,holland2005architecture,knight1986experimental}. 
%There has been proposed many diversification techniques about how to mechanically develop various variants including number representations, register sets, stack direction, and memory layout~\cite{cox2006n, holland2005architecture}. 





%The concept of diversification is also important in socioeconomics, given a strong link between structural network diversity and economic development~\cite{Eagle2010Science}.


%Existing models and analyses of MTD were conducted at lower-level and microscopic abstractions, including analyzing how the attacker's success probability is related to the attacker's time/cost \cite{Maleki:2016:MMM:2995272.2995273}, analyzing the effectiveness of MTD mechanisms from a localized view \cite{DBLP:series/ais/Manadhata13,ZhuGameSec13,DBLP:conf/icc/CarrollCFB14,MonroseOakland13,EvansMTDBookChapter2011,Sovarel:2005:WFE:1251398.1251408,Shacham:2004:EAR:1030083.1030124}, analyzing attack graphs or attack trees in the presence of MTD mechanisms \cite{zhuang2015theory,zhuang2015theory-PhDDissertation,zhuang2014model,6903607,7122306}, algorithmic analysis of attacker's view of a target system \cite{Albanese2016,DBLP:conf/cns/AlbaneseBJC14}, empirical and simulation based analysis \cite{Prakash:2015:EGA:2808475.2808483,Winterrose:2014:SEA:2665049.2665058,DBLP:conf/safeconfig/CrouseF11,Antonatos:2005:DAH:1103626.1103633,IPHopping,BBN-DYNAT,Jafarian:2012:ORH:2342441.2342467}, using MTD for specific purposes \cite{DBLP:conf/ccs/VenkatesanACJ16,DBLP:conf/ccs/WrightVAW16,Li:2016:MTD:2995272.2995286,Chowdhary:2016:SBS:2995272.2995274,Crouse:2015:PPA:2808475.2808480,Xu:2014:CDM:2663474.2663486}, and experimentation of MTD mechanisms \cite{Atighetchi:2016:ESC:2897795.2897812,Taylor:2016:AEE:2995272.2995282,Zaffarano:2015:QFM:2808475.2808476,Alsaleh:2016:TAV:2994475.2994482,Hamlet:2016:DGA:2995272.2995277}.




==> seeking-deeper-insights.tex <==
%Now we seek deeper insights.

%\newpage

%\noindent{\bf Security effectivenss with respect to varying degree of $\zeta$}.
%The degree of software vulnerability can be measured by the prevalence of software vulnerabilities and the attributes of the vulnerabilities, which are respectively investigated below.
We focus on $C_0$ and $C_1$ because $C_0$ in a sense reflects the state-of-the-art and $C_1$ reflects the ideal case.
The other parameters are: $\APP=\{$browser, email client, peer-to-peer (P2P), word processor$\}$, $\KERNEL$= $\OS_1$, $N = 20$, $\gamma = 0.2$, $\alpha = 0.2$, $\vartheta = 0.8$, $\tau = 0.05$, NIPS= $tight$, HIPS= $tight$.
%In the first step, we explore whether network diversity is an effective technique to enhance the network security.
%{\color{red}We simulate two different settings:  of $C$= $\{C_0,C_1\}$, namely using monoculture implementations for each software or enforcing  multi-layer diversity for all softwares.


\begin{figure}[htbp!]
%\setlength{\abovecaptionskip}{0em}
%\setlength{\belowcaptionskip}{-1em}
%\begin{tabular}{cc}
\centering
%\subfigure[$C=C_0$, $\zeta=0.5$]{\label{fig:subfig:a}\includegraphics[width=0.23\textwidth]{./figures/no_diversity.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.5$]{\label{fig:subfig:b}\includegraphics[width=0.23\textwidth]{./figures/diversity_5.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.8$]{\label{fig:subfig:c}\includegraphics[width=0.23\textwidth]{./figures/diversity_3.pdf}}
\subfigure[$C_0$, $\zeta=0.1$]{\label{fig:subfig:a}\includegraphics[width=0.23\textwidth]{./figures/threem_2.pdf}}
\subfigure[$C_1$, $\zeta=0.1$]{\label{fig:subfig:b}\includegraphics[width=0.23\textwidth]{./figures/threem_2_1.pdf}}
\subfigure[$C_0$, $\zeta=0.1$]{\label{fig:subfig:c}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_3.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.8$]{\label{subfig:c}\includegraphics[width=0.23\textwidth]{./figures/kernel_8_1.pdf}}
\subfigure[$C_1$, $\zeta=0.1$]{\label{fig:subfig:d}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_4.pdf}}
\subfigure[$C_0$, $\zeta=0.2$]{\label{fig:subfig:e}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_1.pdf}}
%\subfigure[$C=C_1$, $\zeta=0.8$]{\label{subfig:c}\includegraphics[width=0.23\textwidth]{./figures/kernel_8_1.pdf}}
\subfigure[$C_1$, $\zeta=0.2$]{\label{fig:subfig:f}\includegraphics[width=0.23\textwidth]{./figures/type2_3m_2.pdf}}
\caption{Plots of $\pca$ and $\pcos$.}
% with $N = 20$, $\gamma = 0.2$, $\alpha = 0.2$, $\vartheta = 0.8$, $\tau = 0.05$, $\omega=0.2$.}
\label{diversity_2}
\end{figure}


Fig. \ref{diversity_2} plot $\pca$ and $\pcos$ with respect to attacker capability $\capa$ (the fraction of vulnerabilities for which the attacker has exploits) and time. 
We observe the following. First, Figs. \ref{fig:subfig:a} and \ref{fig:subfig:c} show that monoculture $C_0$ can lead to sudden ``jumps'' in terms of comppromised applications and operating systems, namely that a single vulnerability can cause the compromise of many software. The ``jumps'' are even more significant for bigger $\zeta$ as shown in Fig. \ref{fig:subfig:e} (e.g., $z=0.2$, meaning 20\% software is vulnerable). However, Figs. \ref{fig:subfig:b} and \ref{fig:subfig:d} show that the enforcement of network diversity $C_1$ does not suffer from this problem. This confirms the intuition that diversity can make the damage increases smoothly rather thna abruptly. This example highlights that diversity can make the security degrades gradually rather than abruptly.

Second, suppose $\zeta$ is fixed, meaning that the secuirty quality of independent implementations (in terms of their probabilities of contianing a vulnerability) is the same. Suppose the attacker capability of the attacker $\capa$, namely the number of exploits the attacker has is proportional to the number of vulnerabilities. Figs. \ref{fig:subfig:a} and \ref{fig:subfig:b} show that $\pca(100)$ with repsect to $C_0$ and $\pca(100)$ with respect to $C_1$ are almost the same, meaning that enforcing software diversity does not lead to better security. This is because increasing $N$ also increasing $N\times \zeta \times \capa$ proportionally for fixed $\zeta$ and $\capa$. This example highlights when diversity neither increase nor decreases security.

Third, by comparing Figs. \ref{fig:subfig:b} and \ref{fig:subfig:e}, we observe that diversity indeed leads to higher security when the diversified software has fewer vulnerabilities than the monoculture case. Indeed, the security resulting from diversity is almost proportional to the improvement in software quality, namely the improvement in terms of reducing $\zeta$ (the probability that a software is vulnerable) from 0.2 to 0.1. This example highlights when diversity leads to higher security.

Fourth, by comparing Figs. \ref{fig:subfig:a} and \ref{fig:subfig:f}, we observe that diversity actually can lead to worse security when the software quality in the divresified implementations is lower. Indeed, the security resulting from the use of diversified low-quality software is almost proportional to the quality of the software. For example, considering $\capa=1$ and $t=100$, the damage when using diversified software with $\zeta=0.2$ is, in terms of $\pca$, {\color{red}????} times of the damange when using monoculture with $\zeta=0.1$. This example highlights when diversity actually leads to lower security.

% compromised applications shows a "stepped" increase if there is no network diversity employed. In some interval such as $\capa\in(0.5,0.6)$ the graph is nearly flat which indicates that there is few application being newly compromised. However, in some other interval such as $\capa\in(0.6,0.7)$, a dramatic leap appears, which suggests that a large number of applications are compromised during this period. This phenomenon illustrates that the security state of the network with monoculture softwares is quite unpredictable and highly dependent on the attacker's capability, that is the exploits the attacker own. Once the attacker owns the exploit of a vulnerability existing in the network, all the hosts running this application will be the victims. On the other hand, Figure \ref{fig:subfig:b}, \ref{fig:subfig:d} present relatively smooth surfaces, which indicates that whoever the attacker is or whatever the attacker's capability might be, the security state of the network is predictable to some extent if a multi-layer diversity technique is employed on the network. The scenario that a great many applications/hosts are compromised at the same time will no happen.

%Figure \ref{diversity_2} plots the evolution of compromised operating systems in the network with the increasing of attacker's capability $\capa$ over time. The phenomenon is similar except that the compromised operating systems shows a more obvious "stepped" increase. This illustrates that there may exist several factors contributing to the compromise of applications, not only vulnerabilities in application layer, but also vulnerabilities in library layer and operating system, which make the evolution of compromised applications mitigatory comparing with the evolution of compromised operating systems.

%Besides, Figure \ref{diversity_2} shows that network diversity does not necessarily improve network security. The growing infection rate is closely related to the value of $\zeta$, namely the proportion of vulnerable implementations. To make it clear, Figure \ref{right_views} depicts the right view of each graph in Figure \ref{diversity_1} as an example. As is shown, the pink curve representing monoculture is interlaced with the green curve which represents the diversity with $\zeta$=0.5, always above the blue curve with $\zeta$=0.2 and below the cyan curve with $\zeta$=0.8. This indicates that if the proportion of vulnerable implementations is above 0.5, network security will not be enhanced by diversity, but even reduced in this scenario. However, a lower proportion of vulnerable implementations will lead to a better security state of the network.

%In summary, we have 
\begin{insight}
Network diversity can make the security degrade gradually rather than abruptly. However, the security effectiveness of network diversity largely depends on the quality of the diversified software implementations, meaning that diversity can increase, have no significant impact on, or decrease security depending on the relative quality between the diverisified implementations and the monoculture implementations.
%will definitely avoid the rapidly widespread outbreaks of infection because of software monoculture and make network security state predictable, but does not definitely enhance the network security, which is highly dependent on the proportion of vulnerable implementations.
\end{insight}


\ignore{

\noindent{\bf Security effectivenss with respect to varying $\vartheta$ and $\tau$}.
After considering the most important direct factors in network diversity, we investigate some other factors that might also influence the effectiveness of diversity. First,we consider the impact of software vulnerability attributes, namely attributes $\loc$ and $\zd$ for each vulnerability exits in softwares.  We setup scenario instances studied here take $\APP=\{\text{browser, email client, peer-to-peer (P2P), word processor}\}$, $\KERNEL$= $\OS_1$, $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\zeta=0.2$, $\omega=1$, $\capa=1.0$, $C=C_1$, NIPS= $tight$, HIPS= $tight$.

\begin{insight}
The occupation ratio of vulnerabilities that can be exploited remotely in the network will affect both the compromise rate and convergence speed against applications and operating systems. The occupation ratio of zero-day vulnerabilities
in the network will only affect the convergence speed if there does not exist a HIDS.
\end{insight}
 \begin{figure}[htbp!]
%\setlength{\abovecaptionskip}{0em}
%\setlength{\belowcaptionskip}{-1em}
%\begin{tabular}{cc}
\centering
\subfigure[impact of $\vul$ attribute of $\loc$]{
\label{vul_loc}
\includegraphics[width=0.23\textwidth,height=.2\textwidth]{./figures/loc.pdf}}
\subfigure[impact of $\vul$ attribute of $\zd$]{
\label{vul_zd}
\includegraphics[width=0.23\textwidth,height=.2\textwidth]{./figures/zd.pdf}}
\caption{Plot of $\pca(t)$ and $\pcos(t)$ with $C=C_1$, $N$ = 20, $\gamma$ = 0.2, $\alpha$ = 0.2, $\zeta=0.5$, $\omega=0.2$, $\capa=1.0$,  changing vulnerability attributes $\vartheta$ and $\tau$. }
\label{vul}
\end{figure}

In order to investigate the impact of $\vartheta$, we set $\tau=0.05$ which means that around 5\% vulnerabilities in the network are zero-day vulnerabilities. We observe the evolution of compromised applications and compromised operating systems with different settings of $\vartheta\in\{0,0.5,1.0\}$ as shown in Figure \ref{vul_loc}, the value of $\vartheta$ will affect both the infection speed and final infection rate. To be specific, the higher the proportion of vulnerabilities that can be exploited remotely in the network, the faster and the more applications and operating systems will be compromised. This is owing to the fact that remote exploitation is always the main channel to make lateral movement.

In order to investigate the impact of $\tau$, we fix $\vartheta=1.0$ to observe the evolution of application infection rate with different settings of $\tau\in\{0,0.5,1.0\}$. As we can see from Figure \ref{vul_zd}, a higher proportion of zero-day vulnerabilities will lead to a drastic compromise speed, while the final compromised applications and compromised operating systems remain unaffected. The rapid compromise speed is mainly due to the feature of zero-day vulnerabilities, namely that they can not be prevented by any intrusion prevention system. The main reason why more zero-day vulnerabilities do not cause more applications compromised is on account of the precondition of our scenario, that is there does not exist a HIDS in each computer which means once a application is compromised it will no longer be detected and recovered. On the other hand, $\alpha>0,\gamma>0$ indicates that a attacker can always try many times until breaking through the intrusion prevention system and compromise the node, and the P2P clients make the attacks more intense.

}



